A Flow Model of Neural Networks

Based on a natural connection between ResNet and transport equation or its characteristic equation, we propose a continuous flow model for both ResNet and plain net. Through this continuous model, a ResNet can be explicitly constructed as a refinement of a plain net. The flow model provides an alternative perspective to understand phenomena in deep neural networks, such as why it is necessary and sufficient to use 2-layer blocks in ResNets, why deeper is better, and why ResNets are even deeper, and so on. It also opens a gate to bring in more tools from the huge area of differential equations.

==> test.tex <==
$$
\bma
\bmb
\bmc
\bmd
\bme
\bmf
\bmg
\bmh
\bmi
\bmj
\bmk
\bml
\bmm
\bmn
\bmo
\bmp
\bmq
\bmr
\bms
\bmt
\bmu
\bmv
\bmw
\bmx
\bmy
\bmz
\bmA
\bmB
\bmC
\bmD
\bmE
\bmF
\bmG
\bmH
\bmI
\bmJ
\bmK
\bmL
\bmM
\bmN
\bmO
\bmP
\bmQ
\bmR
\bmS
\bmT
\bmU
\bmV
\bmW
\bmX
\bmY
\bmZ
$$










